Intriguing Properties of Input-dependent Randomized Smoothing

Randomized smoothing is currently considered the state-of-the-art method to obtain certifiably robust classifiers. Despite its remarkable performance, the method is associated with various serious problems such as "certified accuracy waterfalls", certification vs.\ accuracy trade-off, or even fairness issues. Input-dependent smoothing approaches have been proposed with intention of overcoming these flaws. However, we demonstrate that these methods lack formal guarantees and so the resulting certificates are not justified. We show that in general, the input-dependent smoothing suffers from the curse of dimensionality, forcing the variance function to have low semi-elasticity. On the other hand, we provide a theoretical and practical framework that enables the usage of input-dependent smoothing even in the presence of the curse of dimensionality, under strict restrictions. We present one concrete design of the smoothing variance function and test it on CIFAR10 and MNIST. Our design mitigates some of the problems of classical smoothing and is formally underlined, yet further improvement of the design is still necessary.

==> sections/reproducibility.tex <==
Both our theoretical and practical results and experiments are reproducible. In the theoretical part, we provide all the relevant proofs, insights and all the important reasoning. We use public datasets for our experiments and our code contains just public, well-known libraries. The code will be publicly available after the review process. We do not use seeds for stochastic algorithms, but the level of variance is not large enough to obtain qualitatively different results. Upon request, we are willing to provide models trained by us to obtain exactly the same results. 
